Analysis of the Wikipedia Network of Mathematicians

We look at the network of mathematicians defined by the hyperlinks between their biographies on Wikipedia. We show how to extract this information using three snapshots of the Wikipedia data, taken in 2013, 2017 and 2018. We illustrate how such Wikipedia data can be used by performing a centrality analysis. These measures show that Hilbert and Newton are the most important mathematicians. We use our example to illustrate the strengths and weakness of centrality measures and to show how to provide estimates of the robustness of centrality measurements. In part, we do this by comparison to results from two other sources: an earlier study of biographies on the MacTutor website and a small informal survey of the opinion of mathematics and physics students at Imperial College London.

==> notes.tex <==
% Notes on things
\section*{Future Directions}

Can we learn any tricks for others studying Wikipedia?
\begin{itemize}
\item For instance \citet{EALKVS15} appear to derive information about birth date, birth country and gender from Wikipedia pages.  They only use Wikidata to transcribe names between Wikipedia in different  languages.
\item \citet{GMS15} Use wikidata and a java Wikidata toolset.
\item \citet{WGJS15} use DBpedia dataset which is a ``structured version of Wikipedia that provides meta-data for articles''. Is that the same as Wikidata? Looks at gender of subject in biographical articles.
\item \citet{EL16} use Wikidata to look at Scientists.
\end{itemize} 


The following is based on discussions 26/7/18.
\begin{enumerate}
\item Noise Model
\\
Improvements? Assess the quality of links. Measuring properties of links.  That way a better idea of which links to move or rewire in random noise model.

\item Extracting more data from articles
\\
Can we make more use of the text in the Wikipedia articles?  Can we use related Wikidata information.
\textbf{Option: Can someone look at the feasibility of this?}

\begin{enumerate}
\item Basic Text properties
\\ 
Can we get basic text characteristics such as number of word stems or number of unique words?  This is related to Zipf's law and 
\href{https://en.wikipedia.org/wiki/Heaps'_law}{Heap's Law}
\item NLP (natural Language Processing)
\\
We could try to do a bag-of-words analysis such as TSE can do.  However TSE suspects that this is of limited use as large parts of biographies have nothing to do with mathematics.
\\
However Lin suggests he has better methods that might produce something.
\\
\textbf{*** TO DO} Lin will look at these approaches and see if anything useful appears.
\item Wikidata. The panels of key data on the side of the Wikipedia articels appear to come from Wikidata.  If not Wikidata contains similar information.  See other works using WIkipedia/Wikidata for approaches.
\end{enumerate}

\item What are the questions we ask?
\\
Sharpen these up?
\begin{itemize}
\item Who is the most `important' mathematician?
\item How do you assess the uncertainty or robustness of centrality measures in network analysis?
\item Time evolution? We have two times. \\
\textbf{Option: do we derive a new third data set based on today's data?}
\item How do different computer biographies compare with each other and with a real audience survey?
\item How do we analyse Wikipedia articles?
\\
How does our approach differ form that of others?
\item How do we define a mathematician?
\\
\textbf{TO DO} Compare the number of mathematicians in both MacTutor and Wikipedia data sets.
\\
Use fuzzy matching to try to link up names.
\\ 
\textbf{TO DO} Check how mathematical our biographies are. Look at non-mathematicians (a) as suggested by PLOS One  referee 2, (b) by our own random sampling. Pass our own `expert' definition of being a mathematician. Compare with Wikidata classification. What if we look at a biassed sample - maybe only the lower ranked mathematicians are of dubious classification.

\end{itemize}

Some possible conclusions
\begin{enumerate}
\item Who is the most important Mathematician?
\item Detailed compariosn between 2013 and 2017 data
\item General comparison with MacTutor results
\item General discussion of use of Wikipedia to study systems like this
\end{enumerate}

\end{enumerate}
  
\section*{Possible Journals}
  
Check to see if they accept pdf for initial submission, LaTeX, Bibliography Style, Impact Factor or try \href{http://www.scimagojr.com/journalsearch.php}{SJR}, open access and its cost (covered by college). I would probably try one of the first three.
\begin{enumerate}
\item \href{https://www.journals.elsevier.com/social-networks/}{Social Networks} (SJR 2016, 1.7; IF 2016, 2.5, Social Science. 1800USD open access fee, \LaTeX OK. We recommend authors see our green open access page for further information. Authors can also self-archive their manuscripts immediately and enable public access from their institution's repository after a 24 month embargo period. As part of the Your Paper Your Way service, you may choose to submit your manuscript as a single file to be used in the refereeing process. This can be a PDF file or a Word document, in any format or lay-out that can be used by referees to evaluate your manuscript.
\item \href{http://journals.plos.org/plosone/}{PLoS One} (SJR 2016, 1.2) \href{https://www.plos.org/publication-fees}{USD1500}
\item \href{https://academic.oup.com/comnet}{J.Complex Networks} OUP (SJR 2016, 1.4)
\item \href{https://www.journals.elsevier.com/physica-a-statistical-mechanics-and-its-applications}{Physica A}(SJR 2016 0.78)
\item \href{http://www.springer.com/physics/complexity/journal/41109}{Applied Network Science} Springer (SJR unlisted)
\item \href{https://www.cambridge.org/core/journals/network-science}{Network Science} CUP (SJR 2016, 0.12, first year listed, listed under social sciences).  We won't use this as I expect this is to be used on a similar Wikipedia project on Painters by Tim and his PhD student.
\end{enumerate}

% % ************************************************
% \section*{Outline}

% The structure of the article

% \begin{enumerate}
% \item Introduction \& Theory. Possible network visualisation?

% \item Data and Methods
% \begin{enumerate}
% \item Graph analysis platform and visualization tool
% \item Description of Data.  Different years of Wikipedia, how did we find which page was a mathematician?
% \item Method of the graph construction from raw Wikipedia page
% \item Simplification of the graph
% \item Noise simulation for Wikipedia- Preferential attachment argument
% \item General ranking scheme used for different centrality measures
% \item Informal survey
% \end{enumerate}

% \item Results \& Discussion
% \begin{enumerate}
% \item Network parameter with and without noise
% \item Degree centrality measure, data-binning and fat-tailed degree distribution(Might put the best fit result into the appendix)
% \item Closeness centrality measure
% \item Betweenness centrality measure
% \item Eigenvector centrality measure
% \item Pagerank centrality measure
% \item Correlations between different centrality measures
% \item Total ranking with and without noise simulation. TSE to produce graphical representation (cube space \& directed acyclic graph, use \texttt{ratings\_dag.py}) for
% \begin{itemize}
% \item individual measures. Edge from $A$ to $B$ if $M(A,25\%)>M(B,75\%)$ where $M(A,q)$ is the centrality measure result for measure $M$, mathematician $A$ and using the quartile value $q$,
% \item for combined overall result (edge from $A$ to $B$ if $M(A)>M(B)$ for all measures $M$ where $M(A)$ is the result from the actual data for mathematician $A$ and centrality measure $M$.
% \end{itemize}


% \item Result compared with MacTutor
% \item Comparison with Informal Survey
% \end{enumerate}

% \item Conclusion

% Some possible conclusions
% \begin{enumerate}
% \item Who is the most important Mathematician?
% \item Detailed compariosn between 2013 and 2017 data
% \item General comparison with MacTutor results
% \item General discussion of use of Wikipedia to study systems like this
% \end{enumerate}

% \item Appendix

% This is material which may go in an appendix or Supplementary Material section of a journal.
% \begin{itemize}
% \item Place any more technical material here.
% \item Place additional figures here. Can't place everything in main text so place extra ones we have here.
% \item Place additional data tables here.
% \end{itemize}

% \item \texttt{figshare.com}

% Set up an archive on \texttt{figshare.com} for archive of files and data that others can use.  Leads to more citations for main paper. A key point here is that we would like to have a UNIQUE id number (a ``CLE-id'') to help ensure all files are coordinated.
% \begin{enumerate}
% \item Basic xml files of Wikipedia pages used
% \item Data representing the graphs used (whole graph and LCC if possible).  \texttt{graphml} is good as it will store  information on the vertices. A \texttt{.net} pajek style file is good as it is pretty universal.
% \item Table of information on vertices. Start with header row then one row for each mathematician.  List things like name, Wikipedia page url, unique id number, and anything we derived, betweennness, degree etc etc. Store as simple \texttt{.xls} excel format file and as tab separated text file.
% \end{enumerate}

% \end{enumerate}

% \section*{Possible Conclusions}

% Some possible conclusions
% \begin{enumerate}
% \item Who is the most important Mathematician?
% \item Comparison between 2013 and 2017 data
% \item General comparison with MacTutor results
% \item General discussion of use of Wikipedia to study systems like this.
% \\
% \href{https://en.wikipedia.org/wiki/Criticism_of_Wikipedia}{General criticisms of Wikipedia} might be useful.
% \\
% \href{https://en.wikipedia.org/wiki/Reliability_of_Wikipedia}{Reliability} of Wikipedia such as the Britanica-Wikipedia comparison paper might be useful background.
% \\
% Examples of Oslo statisticians.  Ivor Grattan-Guiness\bnote{This is not Oslo statistician, but he is one of the most popular historian mathematicians}.
% \\
% Bias issues in English Wikipedia:
% \begin{itemize}
% \item western cultural bias.
% \item \href{https://en.wikipedia.org/wiki/Gender_bias_on_Wikipedia}{gender bias} (\url{https://www.technologyreview.com/s/427626/the-worrying-consequences-of-the-wikipedia-gender-gap/} and \url{http://netplexity.org/?p=954},
% \end{itemize}
% \end{enumerate}


\subsection*{More To DO}

More options
\begin{itemize}
\item Someone try to find a Network visualisation. Probably remove less important vertices. Perhaps do at end of writing.

\item Check the data is on figshare and is up to standard.

\item Informal Survey.
\\
Please make the full counts available, i.e.\ a full electronic version of table \ref{tableinformal}. Excel file with name and counts for one mathematician on each row would do, tab separated text file fine too.

\item The robustness of the closeness values for the top ten mathematicians in 2013 as for 2017 in \fref{clobox} (perhaps for appendix). Produce data shown in plot as a table (perhaps for appendix). Ditto other centralities.
    
    
\end{itemize}

Some extra tables
\begin{table}[h]
\centering
\begin{tabular}{l||c|c|c|c|c|c}
Top 35                    & Degree & PageRank & Eigenvector & Betweenness & Closeness & Average \\ \hline \hline
Degree              & 1.00   & 0.98     & 0.74        & 0.78        & 0.36      & 0.96    \\  \hline
PageRank            & 0.98   & 1.00     & 0.61        & 0.84        & 0.40      & 0.94    \\ \hline
Eigenvector         & 0.74   & 0.61     & 1.00        & 0.46        & 0.34      & 0.80    \\ \hline
Betweenness         & 0.78   & 0.84     & 0.46        & 1.00        & 0.74      & 0.87    \\ \hline
Closeness           & 0.36   & 0.40     & 0.34        & 0.74        & 1.00      & 0.57    \\ \hline
Average             & 0.96   & 0.94     & 0.80        & 0.87        & 0.57      & 1.00
\end{tabular}
\caption{The Pearson correlation values for the 35 top mathematicians (by the average of centrality scores). Note that degree and PageRank are particularly well correlated as are Betweenness and Closeness.}
%Based on TSE Excel calcualtion from score17.xlsx, using score17numbers35.xlsx and  http://www.tablesgenerator.com/latex_tables
\label{tPearson35}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{l||c|c|c|c|c|c}
Top 35             & Degree & Betweenness & Closeness & Eigenvector & PageRank & Average  \\ \hline \hline
Degree                  & 1.00            & 0.55                 & 0.28               & 0.63                            & 0.92                         & 0.88          \\ \hline
Betweenness    & 0.55            & 1.00                 & 0.77               & 0.23                            & 0.71                         & 0.71          \\ \hline
Closeness               & 0.28            & 0.77                 & 1.00               & 0.33                            & 0.30                         & 0.58          \\ \hline
Eigenvector& 0.63            & 0.23                 & 0.33               & 1.00                            & 0.39                         & 0.76          \\ \hline
PageRank     & 0.92            & 0.71                 & 0.30               & 0.39                            & 1.00                         & 0.80          \\ \hline
Average & 0.88            & 0.71                 & 0.58               & 0.76                            & 0.80                         & 1.00
\end{tabular}
\caption{The Spearman correlation values for the 35 top mathematicians (by the average of centrality scores). Note that degree and PageRank are particularly well correlated as are Betweenness and Closeness.}
%Based on TSE Excel calculation from score17.xlsx, using score17numbers35.xlsx and  http://www.tablesgenerator.com/latex_tables
\label{tSpearman35}
\end{table}

\clearpage

\newpage

